Tight Lower Bounds for Planted Clique in the Degree-4 SOS Program

We give a lower bound of $\tilde{\Omega}(\sqrt{n})$ for the degree-4 Sum-of-Squares SDP relaxation for the planted clique problem. Specifically, we show that on an Erd\"os-R\'enyi graph $G(n,\tfrac{1}{2})$, with high probability there is a feasible point for the degree-4 SOS relaxation of the clique problem with an objective value of $\tilde{\Omega}(\sqrt{n})$, so that the program cannot distinguish between a random graph and a random graph with a planted clique of size $\tilde{O}(\sqrt{n})$. This bound is tight. We build on the works of Deshpande and Montanari and Meka et al., who give lower bounds of $\tilde{\Omega}(n^{1/3})$ and $\tilde{\Omega}(n^{1/4})$ respectively. We improve on their results by making a perturbation to the SDP solution proposed in their work, then showing that this perturbation remains PSD as the objective value approaches $\tilde{\Omega}(n^{1/2})$. In an independent work, Hopkins, Kothari and Potechin [HKP15] have obtained a similar lower bound for the degree-$4$ SOS relaxation.

==> tikzdrawings/diamonds.tex <==
\begin{tikzpicture}[scale = 0.75]
    \def\hspc{2}
    \def\vspc{0.7}
    \def\shift{6}
\draw (\hspc, -\vspc) node[circle,fill=white] (d) {$d_j$}
--(0,0) node[circle,fill=white] (i) {$i_j$}
-- (\hspc, \vspc) node[circle,fill=white] (c) {$c_j$};
\draw (-\hspc, -\vspc) node[circle,fill=white] (b) {$b_j$}
-- (i)
-- (-\hspc, \vspc) node[circle,fill=white] (a) {$a_j$};
%---------------
\draw (\shift+ \hspc, -\vspc) node[circle,fill=white] (d2) {$d_{j+1}$}
--(\shift,0) node[circle,fill=white] (i2) {$i_{j+1}$}
-- (\shift + \hspc, \vspc) node[circle,fill=white] (c2) {$c_{j+1}$};
\draw (\shift-\hspc, -\vspc) node[circle,fill=white] (b2) {$b_{j+1}$}
-- (i2)
-- (\shift -\hspc, \vspc) node[circle,fill=white] (a2) {$a_{j+1}$};
\draw[dashed] (c) -- (a2);
\draw[dashed] (d) -- (b2);
\draw[dashed] (c2) -- (\shift + \hspc + 1,\vspc);
\draw[dashed] (d2) -- (\shift + \hspc + 1,-\vspc);
%---------------
\draw (-\shift+ \hspc, -\vspc) node[circle,fill=white] (d0) {$d_{j-1}$}
--(-\shift,0) node[circle,fill=white] (i0) {$i_{j-1}$}
-- (-\shift + \hspc, \vspc) node[circle,fill=white] (c0) {$c_{j-1}$};
\draw (-\shift-\hspc, -\vspc) node[circle,fill=white] (b0) {$b_{j-1}$}
-- (i0)
-- (-\shift -\hspc, \vspc) node[circle,fill=white] (a0) {$a_{j-1}$};
\draw[dashed] (a) -- (c0);
\draw[dashed] (b) -- (d0);
\draw[dashed] (a0) -- (-\shift - \hspc - 1,\vspc);
\draw[dashed] (b0) -- (-\shift - \hspc - 1,-\vspc);
%------------------
\draw[very thick] (-1.2*\hspc,- \vspc - 0.5)--(-1.1*\hspc,- \vspc - 0.7) -- (1.1*\hspc,-\vspc-0.7) -- (1.2*\hspc,- \vspc - 0.5);
\end{tikzpicture}


==> tikzdrawings/iso-paths.tex <==
\begin{tikzpicture}[scale = 0.75]
    \def\spc{6}
    \def\ispc{2}
    \draw
    (-\ispc - \spc,0) node[circle,fill=white] (b0) {$b_{j-1}$}
    -- (0 - \spc,0) node[circle,fill=white] (i0) {$i_{j-1}$}
    -- (\ispc- \spc,0) node[circle,fill=white] (c0) {$c_{j-1}$};
    \draw (0- \spc,0.7*\ispc) node[circle,fill=white] (a0) {$a_{j-1}$};
    \draw
    (-\ispc,0) node[circle,fill=white] (b) {$b_j$}
    -- (0,0) node[circle,fill=white] (i) {$i_j$}
    -- (\ispc,0) node[circle,fill=white] (c) {$c_j$};
    \draw (0,0.7*\ispc) node[circle,fill=white] (a) {$a_j$};
    \draw
    (-\ispc + \spc,0) node[circle,fill=white] (b2) {$b_{j+1}$}
    -- (0 + \spc,0) node[circle,fill=white] (i2) {$i_{j+1}$}
    -- (\ispc+ \spc,0) node[circle,fill=white] (c2) {$c_{j+1}$};
    \draw (0+ \spc,0.7*\ispc) node[circle,fill=white] (a2) {$a_{j+1}$};
    \draw[dashed] (a0) -- (b);
    \draw[dashed] (b2) -- (c);
    \draw[very thick] (-1.2*\ispc, - 0.5)--(-1.1*\ispc, - 0.7) -- (1.1*\ispc,-0.7) -- (1.2*\ispc, - 0.5);
\end{tikzpicture}

